Persistent Homology for Labeled Datasets: Gromov-Hausdorff Stability and Generalized Landscapes

Techniques from metric geometry have become fundamental tools in modern mathematical data science, providing principled methods for comparing datasets modeled as finite metric spaces. Two of the central tools in this area are the Gromov-Hausdorff distance and persistent homology, both of which yield isometry-invariant notions of distance between datasets. However, these frameworks do not account for categorical labels, which are intrinsic to many real-world datasets, such as labeled images, pre-clustered data, and semantically segmented shapes. In this paper, we introduce a general framework for labeled metric spaces and develop new notions of Gromov-Hausdorff distance and persistent homology which are adapted to this setting. Our main result shows that our persistent homology construction is stable with respect to our novel notion of Gromov-Hausdorff distance, extending a classic result in topological data analysis. To facilitate computation, we also introduce a labeled version of persistence landscapes and show that the landscape map is Lipschitz.

==> tikz/interleaving_11.tex <==
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRAHUAKAJwEoQAvqXSZc+QigBM5KrUYs2XbgHJ+QkdjwEiAVhnV6zVog48A1AB0LMNNgYE1wkBk3iiAdn1yjinssvWtlj2YI4aYtooAIykUbKGCibsyuZWNnYOgk4uERLIAMyx8fLGHCkqAenBmerOolp5ACxFBiWK5WF1rpHIAGwt3ollfmqyMFAA5vBEoABm3BAAtkhkIDgQSM2DpVYA7liweAywwFZoABZYAgD63CDUDHQARjAMAAr1biYMMLM4WXMFstEKt1kgYttfNwztwYABjOFMbgMACeMAAjgACFT8B7PV4fboSEA-P4AkDzJbg6hgxB6SEmPYHGBHE5nS43YAqAT3En496fSIk37-WqU4HSNYbRCFBmmbiVIIhTEw+GI5ForEVNJKzJ4l4ColsUmipzizY06X0hKlZKpQIZMAqixoWEIpGojHY-w6x24vkGwm5Y0i8nmxD9KVISU2thMw7BNku7A3O76gmC4kmsNApCR2meOV27jO11qj2a73+x6BzMhsli3OIQu02WxxkWfYJ44wU7Jq7XLnKHnpw3B76hgQUARAA
\begin{tikzcd}
W(r) \arrow[rd, "\widetilde{\phi}_r"] \arrow[rr, "W(r\preccurlyeq r')"] &                                                                      & W(r') \arrow[rd, "\widetilde{\phi}_{r'}"] &                 &                                                                            & W(r+\epsilon) \arrow[rr, "W(r+\epsilon \preccurlyeq r'+\epsilon)"] &                                            & W(r'+\epsilon) \\
                                                                        & W'(r+\epsilon) \arrow[rr, "W'(r+\epsilon \preccurlyeq r'+\epsilon)"] &                                           & W'(r'+\epsilon) & W'(r) \arrow[ru, "\widetilde{\psi}_r"] \arrow[rr, "W'(r \preccurlyeq r')"] &                                                                    & W'(r') \arrow[ru, "\widetilde{\psi}_{r'}"] &               
\end{tikzcd}

==> tikz/interleaving_1_tikz.tex <==
\begin{tikzcd}
{V(r,p)} \arrow[rd, "{\phi_{r,p}}"] \arrow[rr, "{V((r,p)\preccurlyeq (r', p'))}"] &                                                                                      & {V(r',p')} \arrow[rd, "{\phi_{r',p'}}"] &                      &                                                                                     & {V(r+\epsilon,p)} \arrow[rr, "{V((r+\epsilon,p)\preccurlyeq (r'+\epsilon, p'))}"] &                                         & {V(r'+\epsilon, p')} \\
 & {V'(r+\epsilon, p)} \arrow[rr, "{V'((r+\epsilon,p)\preccurlyeq (r'+\epsilon, p'))}"] &                                        & {V'(r'+\epsilon, p')} & {V'(r,p)} \arrow[ru, "{\psi_{r,p}}"] \arrow[rr, "{V'((r,p)\preccurlyeq (r', p'))}"] &                                                                                   & {V'(r',p')} \arrow[ru, "{\psi_{r',p'}}"] &                     
\end{tikzcd}


==> tikz/interleaving_22.tex <==
% https://tikzcd.yichuanshen.de/#N4Igdg9gJgpgziAXAbVABwnAlgFyxMJZABgBpiBdUkANwEMAbAVxiRAHUAKAJwEoQAvqXSZc+QigBM5KrUYs2XbgGpJAHTUw02BgX5CR2PASIAWGdXrNWiDj2UatOvYOEgMR8UQCMpb7KsFW3YAcntHbSxdMH03DzETFABmPwD5Gw4wvldDBIlkAFZUy3TFLNUI5xjBWRgoAHN4IlAAM24IAFskMhAcCCRfOWtFHgACDTRuGABjaaZuBgBPGABHUZV1TUjo-moGOgAjGAYABVFjCRAGGBacHJA2zu7qPqQUoaCQDQB3LFg8BiwYATAAWWAEAH1gNwBCA9odjmdPIkrjc7gYHu0uohpL1+ogih8Mj8-jAAUDQeCoSpKlECLD4UdTucvLZrrd7o9se9XohBoFiWpfv8ohS1JFIdCHFsqgyrgjmcjLuz0W4uUhzHikLiBWwSSLATBgeLsJKYXD5UykXk2CrOViNS98YTdcEsuNxVNZvMlqt1hUZXTqozESyUXaBBQBEA
\begin{tikzcd}
W(r) \arrow[rr, "W(r \preccurlyeq r+2\epsilon)"] \arrow[rd, "\widetilde{\phi}_{r}"] &                                                            & W(r+2\epsilon) &                                                                                       & W(r+\epsilon) \arrow[rd, "\widetilde{\phi}_{r+\epsilon}"] &                 \\
                                                                                    & W'(r+\epsilon) \arrow[ru, "\widetilde{\psi}_{r+\epsilon}"] &                & W'(r) \arrow[ru, "\widetilde{\psi}_{r}"] \arrow[rr, "W'(r \preccurlyeq r+2\epsilon)"] &                                                           & W'(r+2\epsilon)
\end{tikzcd}
